Reconciling interoperability with efficient Verification and Validation within open source simulation environments

A Cyber-Physical System (CPS) comprises physical as well as software subsystems. Simulation-based approaches are typically used to support design and Verification and Validation (V&V) of CPSs in several domains such as: aerospace, defence, automotive, smart grid and healthcare. Accordingly, many simulation-based tools are available, and this poses huge interoperability challenges. To overcome them, in 2010 the Functional Mock-up Interface (FMI) was proposed as an open standard to support both Model Exchange (ME) and Co-Simulation (CS). Models adhering to such a standard are called Functional Mock-up Units (FMUs). FMUs play an essential role in defining complex CPSs through, e.g., the SSP standard. Simulation-based V&V of CPSs typically requires exploring different scenarios (i.e., exogenous CPS input sequences), many of them showing a shared prefix. Accordingly, the simulator state at the end of a shared prefix is saved and then restored and used as a start state for the simulation of the next scenario. In this context, an important FMI feature is the capability to save and restore the internal FMU state on demand. Unfortunately, the implementation of this feature is not mandatory and it is available only within some commercial software. This motivates developing such a feature for open-source CPS simulation environments. In this paper, we focus on JModelica, an open-source modelling and simulation environment for CPSs defined in the Modelica language. We describe how we have endowed JModelica with our open-source implementation of the FMI 2.0 functions to save and restore internal states of FMUs for ME. Furthermore, we present results evaluating, through 934 benchmark models, correctness and efficiency of our extended JModelica. Our results show that simulation-based V&V is, on average, 22 times faster with our get/set functionality than without it.

==> 10-introduction-content.tex <==
%!TEX root = root.tex
\Acp{CPS} integrate physical (\eg mechanical, electrical, etc.) and software
(\eg
\Aclp{SDR}, \Acsp{SDR},
\AcronymUsed{SDR}%
control software, etc.) subsystems.
\Acp{CPS} are widely used in several fields like aerospace, smart grid, manufacturing, automotive, robotics, and health-care (see, \eg \cite{liu2017review,lee2008cyber,rajkumar2010cyber,lee2015cyber,ding2019survey,hayes-etal:2016:tsg,mancini-etal:2014:fmcad,calabrese-etal:2019:rcra,haque2014review}).
As they couple the discrete and continuous dynamics of software and physical subsystems, respectively, \Acp{CPS} are typically defined by means of hybrid systems (see, \eg~\cite{alur:2011:emsoft}).
Due to such a complex nature of \Ac{CPS} models, simulation-based approaches are \emph{typically} used to support design and \Ac{VV} activities.
\Ac{VV} aims at checking whether the \Ac{CPS} model behaviour
satisfies given specifications, \eg safety properties (see, \eg~\cite{nigro2018qualitative,agha-etal:2018:smc-survey}).
In the literature, there are \emph{many} examples where \Ac{VV} activity is performed by means of numerical simulations (see, \eg~\cite{clarke-etal:2010:probabilistic,bogdoll-etal:2012:modest,wang2012hardware,montazeri2012actuator,
duggirala-etal:2015:c2e2,zuliani-etal:2013:fmsd,abbas-etal:2013:tecs} and \cite{kapinski-etal:2016:ver-simulation} for a survey).

Many simulation-based software tools are available to support \Ac{CPS} design such as, \eg AUTOSAR, Automation Studio, AVL Cruise, CATIA, ControlBuild, Simulink, dSpace, EnergyPlus, IBM Rational Rhapsody, ICOS, IGNITE, Dymola, JModelica, MapleSim, Ptolemy II and Virtual Engine.
On one side, the increasing availability of those software tools enables designers to choose the tool chain that best suits their needs.
On the other side, such an availability poses huge interoperability (model exchange) and integration (co-simulation) challenges between \Acp{CPS} modelled using different languages and/or tools.

Furthermore, since physical and/or software subsystems are \emph{usually} designed by different companies (\eg
\Aclp{OEM}, \Acsp{OEM}),
\AcronymUsed{OEM}%
it is also crucial to preserve \Ac{IP} (see, \eg~\cite{durling-etal:2017:fmi-ipp,wekerle-etal:2018:ipp,martinez-etal:2019:ipp}).
As a result, even carrying out simulations of those models may pose problems.

To overcome such interoperability problems, a standardised format, namely, \Ac{FMI}, has been proposed in 2010 as an open standard.
Models adhering to \Ac{FMI} are called \Acp{FMU}.
The current version, \ie \Ac{FMI} 2.0, enables both \Ac{ME} and \Ac{CS}.
\Ac{ME} refers to,
\eg the usage of \Acp{FMU} within different simulation environments,
while \Ac{CS} refers to,
\eg the distributed simulation of heterogeneous systems coupling together several \Acp{FMU}.
Recently, another standard has been defined, \ie \Ac{SSP}, to describe relationships among systems of interconnected \Acp{FMU} and their parametrisation in order to be used in different simulation environments~\cite{sspstandard}.

Typically, simulation-based \Ac{VV} of \Acp{CPS} requires exploring different simulation scenarios, \ie sequences of controllable and/or uncontrollable exogenous inputs.
In this setting, to avoid simulating many times a common prefix of different scenarios, the simulator state is saved in order to be restored later as a start state.
This improves efficiency of simulation-based \Ac{VV} approaches by simulating only once the same prefix of different simulation scenarios (see, \eg~\cite{mancini-etal:2016:micpro} and citations thereof).

Not only \Ac{VV} approaches benefit from such an optimization, but also, \eg
approaches for the automated synthesis of plans/control strategies
such as \cite{margellos-etal:2010:simulation-mpc,ascione-etal:2016:mpc-simulation,aftab-etal:2017:mpc-simulation,dias-etal:2018:mpc-simulation} where simulation-based \Ac{MPC} methods are used and \cite{mpc-pbpkpd,sinisi-etal:2020:fundamenta} where a pharmacological treatment strategy is automatically designed by means of simulations.

To this end, modern simulators (such as, \eg Simulink~\cite{simulink}) offer their own \Ac{API} allowing to save and restore the internal simulator state on demand.
As well as the other simulators, the \Ac{FMI} 2.0 \Ac{API} specifies a way of saving and restoring internal \Ac{FMU} states.
This feature is crucial to increase efficiency of simulation-based \Ac{VV}.

Unfortunately, the implementation of such a feature is not mandatory according to \Ac{FMI} 2.0 specifications.
Hence, even if the \Ac{FMI} standard is currently adopted by several modelling environments (see \cite{fmitools} for a full list) only a few commercial software implement this feature within their generated \Acp{FMU}.

Among them we note Dymola, a state-of-the-art modelling and simulation environment~\cite{dymola},
that is based on Modelica~\cite{modelica}, an open-standard language for modelling dynamical systems.

Modelica is an object-oriented, equation-based language for model-based development.
Moreover, it allows the definition of complex dynamical systems as a network of
smaller subsystems.
Currently, Modelica is widely used by many companies and it is adopted by several simulation environments:
commercial (\eg SimulationX~\cite{simulationx} and SystemModeler~\cite{systemmodeler})
as well as
open source (\eg Open Modelica~\cite{openmodelica} and \JModelica~\cite{jmodelica}).
However, none of the currently available open-source Modelica environments
implement the \Ac{FMI} 2.0 optional feature for saving and
restoring \Ac{FMU} states.
As a result, the interoperability enabled by the \Ac{FMI} standard cannot be fully exploited for \Ac{VV} when using those open-source environments.

This motivates developing such a feature for Modelica-based and open-source CPS simulation environments.

In the literature the save-and-restore feature has been widely exploited for formal verification both for finite state systems (see, \eg~\cite{holzmann1997model,holtzmann:2012:parallel-spin,dill1992protocol,dellapenna-etal:2004:sttt}) as well as, in a simulation-based framework, for \Acp{CPS} (see, \eg~\cite{mancini-etal:2013:cav,mancini-etal:2015:sylvaas-pdp,mancini-etal:2016:micpro}). We refer the readers to those references and citations therein for general considerations and more details about algorithms that exploit such a feature.

In this paper, we provide methods and tools to implement \Ac{FMI} 2.0
functionalities that save and restore the
internal \Ac{FMU} state for \Ac{ME} \Acp{FMU} and we focus on \JModelica modelling and simulation environment.

Furthermore,
we present experimental results to evaluate the correctness of our proposed implementation. Finally, we also conduct an analysis of performance
focusing on \Ac{VV} approaches that drive given \Acp{FMU} by means of simulations.
To do so, we analyse $\totalFMUpass$ \Acp{FMU} generated from benchmarks models taken from widely-used repositories and we show that,
using our tool,
a \Ac{VV} activity in the style of~\cite{mancini-etal:2013:cav} is, on average, $\TotalAvgSpeedup$ times faster than without it.


We remark that  
such a proposed implementation closes an important gap between commercial and open-source Modelica environments.
Indeed, it enables
the application of the above-mentioned 
simulation-based \Ac{VV} approaches to \Acp{CPS} modelled within open-source Modelica environments.
Furthermore, it also fosters the
development of new approaches.

Moreover, the aim of this paper is also to encourage developers of open-source simulation environments to implement modern functionalities of current \Ac{FMI} specifications;
and to push towards future \Ac{FMI} specifications that include a mandatory implementation of such functionalities.
For these reasons,
our proposed implementation is free and \emph{publicly available} at the following repository: \RepoUrl, as a fork of the \JModelica \JModelicaVersion open-source distribution, which is developed by Modelon\footnote{\url{https://www.modelon.com}} and currently available upon request.


The paper is organised as follows.
\cref{sec:related-work} discusses related work.
\cref{sec:methods} describes our methodology to implement get/set \Ac{FMU} state functionality and to evaluate correctness and performance of the proposed implementation.
\cref{sec:results} presents experimental results.
Finally, \cref{sec:conclusions} draws conclusions.



==> 15-related-work-content.tex <==
%!TEX root = ./root.tex
The \Ac{FMI} is a widely used standard for model-based design and analysis of \Acp{CPS}. In the literature we find many examples in different fields (see, \eg \cite{jensen2017integrating,vcech2017novel,cremona2016step,gomes2019semantic}).
Both \Ac{CS} and \Ac{ME} paradigms are crucial to handle large-scale systems (see, \eg \cite{thule2019maestro,falcone2019distributed}).
The former is needed to integrate and analyse in a distributed fashion different subsystems having different characteristics as, \eg the embedded solver needed to simulate the model (see, \eg \cite{gomes-etal:2018:acm-comp-survey,schweiger-etal:2019:cs-survey} for recent surveys).
The latter is used to, \eg import and/or export models as black-box objects among different simulation environments in order to analyse and simulate them with different solvers.
As anticipated in \cref{sec:intro}, we focus on Modelica-based open-source platforms compliant with the last version of \Ac{FMI} for \Ac{ME}, namely 2.0.

Several commercial and open-source modelling and simulation environments support \Ac{FMI} 2.0 (more than 100, see~\cite{fmitools} for a full list).

Among commercial environments, we note Matlab/Simulink~\cite{simulink}: a widely-used and well-known platform for model-based design.
It also offers its own \Ac{API} for advancing forward and backward the simulation by rolling back simulator states (thanks to a save/restore functionality). 
However, being a commercial software, Simulink supports only export of \Acp{FMU} for \Ac{CS} and does not implement get/set functionality of \Ac{FMI} 2.0.

The \Ac{FMI} standard is supported also by some major Modelica-based commercial modelling and simulation environments such as:
\begin{enumerate}
    \item Dymola 2020~\cite{dymola}, which, to the best of our knowledge, is the only Modelica-based modelling and simulation platform \emph{fully} implementing \Ac{FMI} 2.0 standard.
    Hence, it generates \Acp{FMU} for \Ac{CS} and also for \Ac{ME} having get/set state functionality implemented. 
    \item SystemModeler 12~\cite{systemmodeler}, which allows users to generate their models as \Acp{FMU} for both \Ac{CS} and \Ac{ME}. However, no \Ac{FMU} get/set state functionality is implemented.
    \item SimulationX 4.1~\cite{simulationx}, which also provides an implementation to get/set state functionality. However such a functionality is enabled only within \Acp{FMU} for \Ac{CS}.
\end{enumerate}

As motivated in \cref{sec:intro}, we focus on open-source modelling and simulation environments.
\begin{table}
    \centering
    \begin{tabular}{ccc}
    \toprule
    \multirow{2}{*}{Tool} & \multirow{2}{*}{Modelica Support} & \multirow{2}{3cm}{\centering Get/Set \Acs{FMU} state functionality}\\% & \multirow{2}{*}{License}\\
    & &\\% &\\
    \midrule

    DACOSSIM & - & -\\
    FMI4J & - & -\\% 
    QTronic FMUSDK & - & -\\
    \JModelica & \textbullet & -\\
    OpenModelica & \textbullet & -\\
    PythonFMU & - & -\\
    Simulix & - & -\\
    Reference FMUs & - & \Acs{ME} \& \Acs{CS}\\
    \midrule
    \multirow{2}{3cm}{\centering Our extended \JModelica} & \multirow{2}{*}{\textbullet} & \multirow{2}{*}{\Acs{ME}}\\
    & &\\% &\\
    \bottomrule
    \end{tabular}
    \caption{Open source modelling and simulation environments supporting \Ac{FMI} 2.0.}
    \label{table:fmi-comparison}
\end{table}

In \cref{table:fmi-comparison} we compared several open-source platforms which support \Ac{FMI} 2.0.
We split these platforms in the following groups:
\begin{enumerate}
    \item The first group consists of all modelling and simulation environments supporting Modelica.
    Among those, we note OpenModelica~\cite{openmodelica} developed by the Open Source Modelica Consortium.
    OpenModelica translates Modelica models into C code, which, in turn, is compiled in a black-box executable format. Only upon user request it is also possible to wrap such a format into an \Ac{FMU}.
    Conversely, JModelica is \Ac{FMI}-based. Indeed, it directly generates \Acp{FMU} from the input Modelica code. Hence, \Acp{FMU} are first-class citizens.
    This is the main reason why we focus on JModelica. However, we would like to clarify that, with a little effort, our proposed methodology can be quickly adapted to OpenModelica as well.
    \item The second group consists of all modelling and simulation environments which support \Ac{FMI} 2.0 but are not based on Modelica.
    Among those, \emph{Reference FMUs}~\cite{referencefmu} implements get and set of \Ac{FMU} states. However, besides the fact that it is not Modelica-based, this software is just a small tool used for debugging \Acp{FMU}.
\end{enumerate}

A work close to ours is the NANDRAND simulation platform~\cite{nandrand} which provides and simulates ready-to-use models to measure energy performance of physical buildings. Such models can be exported as \Acp{FMU} compliant to \Ac{FMI} 2.0 and support get/set state functionality.
It is worth noting that NANDRAND imports external \Acp{FMU} (\eg generated by a Modelica-based environment) and couples them to NANDRAND models in a \Ac{CS} setting.
However, as the authors specify, such a use-case works if and only if the imported \Acp{FMU} support state saving and restoring.

Another tool related to our work is the {FMI++ library}~\cite{widl-etal:2013:fmi++} which is useful to simulate \Acp{FMU} for \Ac{ME}. One of the features implemented by this library is a wrapper class, called \texttt{RollbackFMU}. Such a class stores, at each integration step, the current state of the input \Ac{FMU} in order to enable a rollback functionality.
The functions used to save and restore the state are \texttt{fmi2GetContinuousState} and \texttt{fmi2SetContinuousState}, respectively.
However, as \Ac{FMI} specifications clarify, such functions are not intended to set and get the complete FMU state but just values of continuous variables of the given \Ac{FMU}.
As \cref{sec:state-architecture} describes in details, this is not enough. The state of an \Ac{FMU} has a complex structure where values of continuous model variables are just a small fraction of it.




==> 20-methods-algo-content.tex <==
%!TEX  root=root.tex
\begin{algorithm}
  % \DontPrintSemicolon
  \SetKwFunction{EvalCorr}{evaluateCorrectness}
  \Fn{\EvalCorr{}}{
    \KwIn{\Acs{FMU}}
    \KwIn{$\tau$, simulation duration}
    \KwIn{$\varepsilon \in (0,1)$}
    \KwIn{$\delta \in (0,1)$}
    \KwIn{$\mathbb{B} \subset \RealsGEZ$}
    \KwOut{either $(\texttt{True}, -, -)$ or a counterexample $(\texttt{False}, \tau', i)$}
    \AlgoVarGets{N}{$\left\lceil\frac{\log{(\delta)}}{\log{(1-\varepsilon)}}\right\rceil$}\;
    \tcc{$H_0 = \Pr\{\tau' \in \mathbb{B} \,.\, \simulate{\tau} \neq \simulatemod{\tau}{\tau'}\} \geq \varepsilon$}
    \For{$i \in \left[1, N \right]$}{
      \AlgoVarGets{$\tau'$}{$\texttt{rand($\mathbb{B}$)}$}\;
      \AlgoVarGets{$s_i$}{$\simulate{\tau}$}; \AlgoVarGets{$s$}{$\simulatemod{\tau}{\tau'}$}\;
      \If{$s_i \neq s$}{\label{algo:line:neq}
        \Return $(\texttt{False}, \tau', i)$ \tcc{$H_0$ is proved}
      }
    } 
    \Return $(\texttt{True}, -, -)$ \tcc{$H_0$ is rejected}
  }
\caption{Hypothesis testing approach to evaluate correctness of \fmiSet and \fmiGet.}
\label{algo:correctness}
\end{algorithm}


==> 20-methods-content.tex <==
%!TEX root = root.tex
In this section, first, we introduce \Ac{FMI} 2.0 for \Ac{ME} with a particular emphasis on \JModelica \Ac{FMU} implementation. Second, we describe the steps needed to enable saving and restoring of internal \Ac{FMU} states. Finally, we present our approach to evaluate the correctness of our implementation and to measure performance when adopting such implementation within simulation-based \Ac{VV} methods.

\subsection{FMI 2.0 for Model Exchange}%
\label{sec:fmi}%
\Input{20-methods-fmu-definition.tex}%
%
\subsection{Enable saving and restoring of JModelica FMU internal state}%
\label{sec:state-architecture}%
\Input{20-methods-fmu-architecture.tex}%
\Input{20-methods-fmu-state.tex}%
%
\subsection{Correctness evaluation strategy}%
\label{sec:validation}%
\Input{20-methods-validation.tex}%
%
\subsection{Performance evaluation strategy}%
\label{sec:performance}%
\Input{20-methods-performance.tex}%
%


==> 20-methods-fmu-architecture.tex <==
%!TEX root = ./../root.tex
%
\JModelica generates an \Ac{FMU} starting from a model written in Modelica.
To do so, Modelica equations are translated into C code and compiled to produce an \Ac{FMU}.
The output \Ac{FMU} consists also of a library (the same for all models) implementing the functions of the \Ac{FMI} standard.
In \JModelica, such a library is called \emph{RuntimeLibrary},
and contains also
% 
relevant data structures responsible for the internal \Ac{FMU} state.


==> 20-methods-fmu-definition.tex <==
%!TEX root = root.tex
%
\Ac{FMI} \Ac{ME} 2.0~\cite{blochwitz-etal:2012:modelica}
specifies an interface to the model of a dynamical system defined by
differential, algebraic and/or difference equations.
An executable implementing \Ac{FMI} is called \Ac{FMU}. 
Any simulation environment supporting \Ac{FMI} can simulate an \Ac{FMU} produced
by any modelling environment.
In particular, an \Ac{FMU} is a ZIP archive consisting of the following parts.
First, C code and/or binaries implementing functions defined by the \Ac{FMI}
\Ac{API}.
Second, an \Ac{XML} document with model metadata including, \eg model identifier, names of variables and
capability flags.
The latter allows omitting implementation of non-mandatory
functionalities.
For example,
the \texttt{canGetAndSetFMUstate} and \texttt{canSerializeFMUstate} capability flags
indicate whether \Ac{FMU} supports functionality to save/restore and serialize/deserialize its internal state or not.


==> 20-methods-fmu-state.tex <==
%!TEX root = root.tex

The internal \Ac{FMU} state is a snapshot containing all the information needed
to simulate the \Ac{FMU} starting from the moment when the state was retrieved.

\begin{figure}
  \centering
  \begin{tikzpicture}
    \umlclass[alias=root]{jmi\_t}{
      z : real [1..*]\\
      z\_last : real [1..*]\\
      \ldots\\
      ext\_objs : pointer [0..*]
    }{}
    \umlsimpleclass[alias=delay,x=6]{jmi\_delay\_t}
    % }{}
    \umlsimpleclass[alias=dae,y=3.5]{jmi\_block\_residual\_t}
    \umlsimpleclass[alias=solver,y=5.5]{jmi\_block\_solver\_t}
    \umlsimpleclass[alias=solver-kinsol,x=6,y=4]{jmi\_kinsol\_solver\_t}
    \umlsimpleclass[alias=solver-linear,x=6,y=7]{jmi\_linear\_solver\_t}
    \umlcompo[arg1=delays,pos1=0.4,mult2=0..*]{root}{delay}
    \umlcompo[arg1=dae\_equation\_blocks,align1=bottom,arg2=jmi,mult2=0..*]{root}{dae}
    \umlcompo[arg1=solver,arg2=block,mult2=1]{dae}{solver}
    \umlinherit[geometry=|-]{solver-linear}{solver}
    \umlinherit[geometry=|-]{solver-kinsol}{solver}
    % \umlnote[y=-3]{root}{The ``root'' class modelling an \Ac{FMU} instance}
  \end{tikzpicture}
  \caption{Conceptual \Ac{UML} class diagram of \JModelica \Ac{FMU} implementation.}\label{fig:uml}
\end{figure}

\cref{fig:uml} depicts the conceptual \Ac{UML} class diagram of such \Ac{FMU}
internals focusing on the components of the internal \Ac{FMU} state.
The main class modelling an \Ac{FMU} instance is \texttt{jmi\_t}.
The internal state of a \JModelica \Ac{FMU} is composed of the following
components.

\begin{description}
  \item[Values of model variables.]
    \texttt{jmi\_t} contains several arrays of real values
    (\eg \texttt{z} and \texttt{z\_last})
    to store the information related to the actual values of model variables.

  \item[Delay buffers.]
    Modelica equations can contain occurrences of \texttt{delay(expr,t,tmax)} (\emph{delay operator})
    that return \texttt{expr(time-t)}, \ie the value of
    the expression \texttt{expr} \texttt{t} time units in the past.
    \JModelica implements such an operator by maintaining a buffer
    (\texttt{jmi\_delay\_t}) containing past values of expression \texttt{expr}
    from current time back to \texttt{time}-\texttt{t}.
    the optional argument \texttt{tmax} guarantees an upper bound for the
    buffer size when \texttt{t} is not constant during simulation.
    The buffer size increases until the current time is greater than
    \texttt{t} (\texttt{tmax} when \texttt{t} is variable).
    After that, the size remains constant.
  \item[Internal state of algebraic solvers.]
    Algebraic equations are split into blocks (\texttt{jmi\_block\_residual\_t})
    that can be solved independently.
    Each such block is equipped with an instance of
    a linear (\texttt{jmi\_linear\_solver\_t})
    or
    a non-linear (\texttt{jmi\_kinsol\_solver\_t}) solver.
    These solvers are stateful, so their internal state also makes part of the
    \Ac{FMU} state.
  \item[Internal state of external objects.] Modelica allows to call
    external (\eg defined in C) functions
    (array \texttt{ext\_objs} of function pointers),
    that can have their own state.
    % \texttt{jmi\_t} contains array \texttt{ext\_objs} of pointers to such
    % functions.
    Note that there is no way to retrieve the state of such external objects,
    since they are completely opaque.
    For example, \Ac{MSL} has the CombiTimeTable block that computes its output
    signal by interpolation in a table.
    It is implemented using C functions that read a table from a file
    into an in-memory data structure and allow to query its values.
    From the \JModelica \Ac{FMU} \emph{RuntimeLibrary} perspective, such data structure
    is just an opaque pointer and there is no way to access it.
\end{description}

Note that, since the above data structures are static, \Ac{FMU} states have a constant size (in bytes).

We extend \JModelica \Ac{FMU} \emph{RuntimeLibrary} by suitably implementing the following \Ac{FMI} functions: 
\begin{itemize}
  \item \fmiGetExtended.
    This method retrieves the current state of a given \Ac{FMU} as an
    in-memory data structure, which is opaque to the user. We refer to this method in the text as \fmiGet.
  \item \fmiSetExtended.
    This method replaces the current state of an \Ac{FMU} with a given \Ac{FMU}
    state previously retrieved using \fmiGetExtended. We refer to this method in the text as \fmiSet.
  \item \fmiFreeExtended.
    This method frees up the memory occupied by a given \Ac{FMU} state retrieved
    using \fmiGetExtended.
  \item \fmiSerializeExtended.
    This method serializes the \Ac{FMU} state retrieved using \fmiGetExtended
    into a byte array that can be stored in a file or sent over the network.
  \item \fmiDeserializeExtended.
    This method deserializes a given byte array into an \Ac{FMU} state that can
    be then passed to \fmiSetExtended.
  \item \fmiSizeExtended.
    This method returns the size of a byte array that is enough to
    serialize a state of the current \Ac{FMU}.
\end{itemize}



==> 20-methods-performance.tex <==
%!TEX root=./root.tex
%
To evaluate performance of our implementation, we focus on simulation-based \Ac{VV} approaches.
As anticipated in \cref{sec:intro}, simulation-based \Ac{VV} of \Acp{CPS} requires to explore all simulation scenarios.
A simulation scenario is a sequence of exogenous inputs to be injected to the given \Ac{CPS} model, \ie \Ac{FMU} under verification.
In this setting, the given \Ac{FMU} (representing the \Ac{CPS} under verification) is driven in the space of all possible simulation scenarios by means of a visit (see, \eg~\cite{mancini-etal:2014:pdp,mancini-etal:2014:dsd-anytime,mancini-etal:2016:fundam} and citations therein).
The space of all simulation scenarios is defined as a tree where each edge is labelled with an exogenous input and 
each node represents the \Ac{FMU} state reached by injecting the sequence of inputs associated to the path leading to that node.

As an example we can consider an FMU defining a simple hybrid system (see, \eg~\cite{alur:2011:emsoft}) having only one state variable.
In particular,
let $x$ be a signal (i.e., a real-valued function of time) and, given a positive real number $T$ (time step), let $u$ be $T$-piecewise constant signal, i.e., 
a signal changing its value only at time instants of the form $kT$ ($k = 0, 1, 2, 3, \ldots$).
In the following we assume that $u$ takes values in the set $\{-1, 1\}$
(i.e., for all $t$, $u(t) \in \{-1, 1\}$).
When writing equations, as usual, we will write $x$ for $x(t)$ and $\dot{x}$ for $\dot{x}(t)$.


Given signals $x$ and $u$ as above, we define the behaviour 
of our simple example of hybrid system by means of the following differential equation:
\begin{align*}
\dot{x} =
\begin{cases} 
-x & \quad \text{if } u \text{ is } -1\\
 x & \quad \text{if } u \text{ is } 1
\end{cases}
\end{align*}
Let $x(0) = 1$ be the initial state of this \ac{FMU} and $2T$ the simulation horizon. \cref{fig:example} depicts all possible simulation scenarios starting from such an initial state and illustrates all state traversed by the \Ac{FMU} when the input function $u(t)$ can change value (i.e., at each $kT$ with $k=0,1,2$). Note that, as described above, states reached by different sequence of inputs (tree paths) are different for us.

\begin{figure}
\centering
  \Input{figures-fmu.tex}
  \caption{Example of a tree of simulation scenarios. Nodes denote \Ac{FMU} states whereas edges denote injected input values.}
  \label{fig:example}
\end{figure}

Typically, the goal of a simulation-based \Ac{VV} activity is to search for an input sequence driving the system to an \emph{undesirable} (error) state (e.g., to verify a safety property stating that \emph{nothing bad} ever happens) or to a \emph{desirable} state (e.g., to verify a liveness property stating that \emph{something good} sooner or later will happen).
Checking a liveness property typically requires looking at the future evolution of the system.
As a result, in general, liveness properties cannot be casted as safety properties (see, e.g.,~\cite{maler2005real}). However, in a bounded horizon setting, such as the one in our simulation-based setting, liveness properties can be casted as safety properties (see, e.g.,~\cite{biere2002liveness,schuppan2006liveness,kupferman2009liveness}) stating that a given state (desirable or undesirable) is reachable, with some suitable input, within the given time horizon. Accordingly, w.l.o.g., we can cast simulation-based \Ac{VV} as the problem of finding an input sequence driving the system to a given state within the given time horizon.

If such a state is not found, the time horizon is increased until an \emph{undesirable} or \emph{desirable} state is found, or some upper bound is reached, namely, the provided simulation horizon $h$ (see, \eg~\cite{fan2015bounded,ren2018simulation}). 
This is equivalent to search for the shortest sequence of exogenous inputs that leads to a given state (see, \eg~\cite{chang2006simulation} and \cite{dill1992protocol,dellapenna-etal:2004:sttt,cimatti1999nusmv} in a finite state context) in the space of all simulation scenarios of length $h$. 
The simulation horizon $h$ is typically set to a value large enough to
guarantee
that,
with high confidence,
the \emph{undesirable} or \emph{desirable state} (if any) is reachable with an input sequence of length at most $h$. To keep $h$ small a \Ac{BFS} is used (\eg as in bounded model checking~\cite{biere2003bounded}).
Furthermore, as anticipated in \cref{sec:intro}, such simulation-based \Ac{VV} approaches are similar to several planning and optimisation approaches such as, \eg~\cite{lipovetzky-etal:2015:ijcai,vallati-etal:2016:aaai,ramirez-etal:2017:ijcai,frances-etal:2017:ijcai,sinisi-etal:2020:fundamenta}, where simulation scenarios and exogenous inputs correspond, respectively, to plans and actions to be taken in order to drive the system into a goal state.

In this setting, in order to decrease the number of simulations and, in turn, the computation time of the \Ac{VV} activity (or the optimisation task), it is important to avoid simulating many times prefixes common to different simulation scenarios.
To do so, it is crucial that the given \Ac{FMU} has the 
save-and-restore state functionality implemented as \Ac{FMU} states can be saved in memory in order to be restored later as initial states of the simulation.


Hence, such an exploration visit in the tree of simulation scenarios is a demanding application to evaluate our proposed implementation.
%
In particular, we distinguish two kind of approaches.
The former uses \Acp{FMU} that are not equipped with the save-and-restore feature of \Ac{FMI} 2.0. We refer to this approach in the text as \traditionalSearch.
The latter is a \optimisedSearch that uses our generated \Acp{FMU} implementing those \Ac{FMI} features to save and restore \Ac{FMU} states.

It is worth noting that during a \optimisedSearch, since the state space to explore can be huge, to keep in memory the whole state space can be infeasible. To this end,
several solutions have been devised in the literature (see, \eg~\cite{mancini-etal:2013:cav,mancini-etal:2015:sylvaas-pdp,mancini-etal:2016:micpro}).
The general idea is to dynamically choose the best states to store and those to forget (compatibly with memory constraints).
% The general idea is to store in memory only those states needed to advance the visit.
Also, whenever no further inputs can be injected from the current node of the tree, the corresponding simulator state can be removed from memory.
We refer the readers to those references for more details and algorithms that efficiently satisfy memory constraints during the visit.
Accordingly, here we focus on evaluating performance of our implementation of the save-and-restore feature in terms of simulation time.

The remainder of this section is organised as follows.
First, we define the space of simulation scenarios of a given \Ac{CPS} model (\ie \Ac{FMU} under verification) as a tree (\cref{sec:search-space}). Second, we show that the time needed to explore such a tree (for both a \traditionalSearch and a \optimisedSearch) strictly depends on the time needed to drive the input \Ac{FMU} through each node of the tree (\cref{sec:trad-search,sec:opt-search}). Last, we quantify the speed-up of a \optimisedSearch (\cref{sec:speed-up}).

\subsubsection{Tree definition}
\label{sec:search-space}
%
In our setting, we perform a visit of a balanced finite tree of depth $\maxHeight > 1$, where each tree node at depth $0 < i \leq h$ has a constant branching factor $\avgBranch > 1$.
% In our setting the search space can be defined as a tree having a height $\maxHeight > 2$ and a branching factor $\avgBranch > 2$.
The tree root corresponds to the initial state of the given \Ac{FMU}, while nodes correspond to \Ac{FMU} states that can be reached through simulations from the initial state.
The edges of the tree correspond to possible actions that can be taken during the visit, \ie different values for the \Ac{FMU} exogenous inputs.
For example, in the tree of \cref{fig:example}, the branching factor, \avgBranch, and the maximum depth, $\maxHeight$, are both $2$.

Furthermore, to simplify calculations, during the visit we assume that the simulation of the input \Ac{FMU} is advanced by a fixed quantity of $\tau \in \RealsGZ$ time units each time a new node is being visited (in our example $\tau$ corresponds to $T$, \ie 1 second).
Also, to simplify our analysis, we assume that the execution time of a simulation depends on the current \Ac{FMU} state and on the simulation duration, \ie $\tau$, and not on values of exogenous inputs.
This might not be strictly true for each simulation, but it is a very reasonable assumption on average for typical \Ac{CPS} models.

\subsubsection{Cost of a \traditionalSearch}%
\label{sec:trad-search}%
A \traditionalSearch aims at driving \Acp{FMU} without get-and-set state capabilities. Hence, when we have to explore a node in the tree, we need to simulate the given \Ac{FMU} from its initial state up to the state denoted by such a node.
% 
This means that a node at depth $i > 0$ can be reached after a simulation of $i\tau$ time units from the initial state of the given \Ac{FMU}. We denote such operation with \simulate{i\tau}.
For example, in \cref{fig:example}, the state $x(2T) = 0.1$ can be reached by means of a $\simulate{2\tau}$ operation, where $\tau = T$, and by injecting $u(0) = -1$ and $u(T) = -1$. 
% 
% 
As already stated in \cref{sec:validation}, \simulate{} can be defined according to \Ac{FMI} 2.0 specifications.

We define our cost function as $\cost{i} = \exectime{\simulate{i\tau}}$, which measures the execution time, $\mathcal{T}$, to reach a node at depth $i > 0$.
Finally, we define the total execution time of a \traditionalSearch as the sum of the costs of each single node in the tree:
\begin{align}
\label{eq:cost-trad}
    \sum_{i=1}^{\maxHeight}{\cost{i}\;\avgBranch^i}
\end{align} 

\subsubsection{Cost of a \optimisedSearch}%
\label{sec:opt-search}%
%
A \optimisedSearch aims at driving \Acp{FMU} by exploiting their get and set capabilities in order to simulate only once each prefix common to different paths of the given tree.
To do so, each time a node at depth $i > 0$ has to be visited, we perform the following steps:
\begin{enumerate}
    \item \fmiSet, to restore (load) the state corresponding to the node at depth $i-1$ as a start state of the given \Ac{FMU};
    \item \simulate{\tau}, to advance the current \Ac{FMU} state to the state reached after a simulation of $\tau$ time units also by injecting the value for exogenous inputs corresponding to the traversed edge.
    \item \fmiGet, to store (save), \eg on disk, the reached \Ac{FMU} state for further steps.
\end{enumerate}
For the sake of readability,
we omit the time needed to perform a \fmiFreeExtended because it is negligible.
\begin{figure}
\centering
  \Input{figures-cost.tex}
  \caption{Usage of \fmiSet and \fmiGet to explore nodes during a \optimisedSearch}
  \label{fig:cost}
\end{figure}
\Cref{fig:cost} outlines the above steps.

As in the previous section, 
we define a cost function, \ie $\costGetSet{i}$, which denotes the execution time spent to visit a node at depth $i > 0$ during a \optimisedSearch, as follows.
\begin{align*}
    \costGetSet{i} = \exectime{\frac{1}{\avgBranch}\;\fmiGet + \fmiSet +
    \simulate{\tau}}.
\end{align*}
Note that the \fmiGet is performed at depth $i-1$ (see \cref{fig:cost}) as the corresponding retrieved \Ac{FMU} state will be then used as a start state for all the children of that node. However, to simplify the formulation we count such \fmiGet time in the child nodes. Hence, each child node (at depth $i$) contributes $\frac{1}{\avgBranch} \fmiGet$ to the total \fmiGet time, \ie the total \fmiGet time is amortised by the branching factor.

Accordingly, along the lines of \cref{eq:cost-trad}, the total execution time needed by a \optimisedSearch to explore the whole tree space is equal to the sum of the costs of each node:
\begin{align}
\label{eq:cost-opt}
    \sum_{i=1}^{\maxHeight}{\costGetSet{i}\;\avgBranch^i}
\end{align}


\subsubsection{Speed-up of a \optimisedSearch}
\label{sec:speed-up}

We define the speed-up, \speedup{\maxHeight}{\avgBranch}, as the ratio between
the cost of a \traditionalSearch, \cref{eq:cost-trad}, and the cost of a \optimisedSearch, \cref{eq:cost-opt}, on a perfectly balanced tree having branching factor $\avgBranch$ and depth $\maxHeight$:
\begin{align}
\label{eq:speed-up}
\speedup{\maxHeight}{\avgBranch} = \frac{\sum_{i=1}^{\maxHeight}{\cost{i}\;\avgBranch^i}}{\sum_{i=1}^{\maxHeight}{\costGetSet{i}\;\avgBranch^i}}
\end{align}

When the above ratio is greater than 1 it means that a \optimisedSearch is faster than a \traditionalSearch.

Furthermore, we note that the above formula, \ie \cref{eq:speed-up}, can be simplified under the following assumptions.

% 
First, the time spent for simulating an \Ac{FMU} for $i\tau$ time units, \ie $\exectime{\simulate{i\tau}}$, is approximately equal to $i \times \avgtime{\simulate{\tau}}$, that is $i$ times the average execution time of a simulation of length $\tau$.

Second, we can use average execution times of \fmiGet and \fmiSet,  \ie \avgtime{\fmiGet} and \avgtime{\fmiSet}, respectively.
As \cref{sec:state-architecture} describes, this is motivated by the fact that states of a given \Ac{FMU} have a constant size (in bytes).

In \cref{sec:results:performance}, we experimentally show that such assumptions are reasonable.

We rewrite $\cost{i}$ as
$\cost{i} = i \times \avgtime{\simulate{\tau}}$
and $\costGetSet{i}$ as
$\costGetSet{i} = \frac{1}{\avgBranch}\;\avgtime{\fmiGet} + \avgtime{\fmiSet} + \avgtime{\simulate{\tau}}$.


Hence, the speed-up of \cref{eq:speed-up}, $\speedup{\maxHeight}{\avgBranch}$, can be written as follows:
\begin{align*}
\speedup{\maxHeight}{\avgBranch} =&
\frac{
\avgtime{\simulate{\tau}} \sum_{i=1}^{\maxHeight}{i\avgBranch^i}
}{
  \left( \frac{1}{\avgBranch}\;\avgtime{\fmiGet} + \avgtime{\fmiSet} + \avgtime{\simulate{\tau}} \right) \sum_{i=1}^{\maxHeight}{\avgBranch^i}
}.
\end{align*}

This leads to the following proposition.

\begin{restatable}{proposition}{propositionspeedup}
\label{prop:speed-up-simple}
Given $\cost{i} = i \times \avgtime{\simulate{\tau}}$
% and
and $\costGetSet{i} = \frac{1}{\avgBranch}\;\avgtime{\fmiGet} + \avgtime{\fmiSet} + \avgtime{\simulate{\tau}}$,
the speed-up of a \optimisedSearch is greater than 1, \ie $\speedup{\maxHeight}{\avgBranch} > 1$, when the following equation is satisfied:
\begin{align}
\label{eq:speed-up-simple}
\frac{
  \frac{1}{\avgBranch}\;\avgtime{\fmiGet} + \avgtime{\fmiSet} 
}{
  \avgtime{\simulate{\tau}}
}
<
\speedupthreshold{\maxHeight}{\avgBranch}
\end{align}
where \speedupthreshold{\maxHeight}{\avgBranch} is a threshold defined as:
\begin{align}
\speedupthreshold{\maxHeight}{\avgBranch} = \frac{
  \sum_{i=1}^{\maxHeight}{i\avgBranch^i}
}{
  \sum_{i=1}^{\maxHeight}{\avgBranch^i}
} - 1 = \frac{
  \maxHeight\avgBranch^{\maxHeight+1} - (\maxHeight + 1)\avgBranch^\maxHeight + 1
}{
  (\avgBranch - 1)(\avgBranch^\maxHeight - 1)
} - 1.
\end{align}
\end{restatable}

\begin{restatable}{remark}{remarklimit}
\label{remark:limit}
When $\avgBranch$ is very large, formally $\avgBranch \rightarrow \infty$, and $\maxHeight > 1$, the speed-up threshold \speedupthreshold{\maxHeight}{\avgBranch} approaches to $\maxHeight - 1$, formally $\speedupthreshold{\maxHeight}{\avgBranch} \rightarrow \maxHeight - 1$.
Thus, \cref{prop:speed-up-simple} can be rephrased saying that $\speedup{\maxHeight}{\avgBranch} > 1$ when the following condition is satisfied.


\begin{align}
\label{eq:speed-up-ratio}
\setsimratio = 
\frac{
  \avgtime{\fmiSet}
}{
  (\maxHeight - 1)  \avgtime{\simulate{\tau}}
}
< 1.
\end{align}
\end{restatable}

Intuitively, \cref{remark:limit} says that when the branching factor of a given tree is sufficiently large and the ratio \setsimratio is less than 1, we expect that the use of get/set state functionality speeds up a \traditionalSearch. Note that, since the \fmiGet is executed once for each node of the tree and the retrieved state is then used as many times as the value of the branching factor $\avgBranch$ of that node (\ie for each child node), the inefficiency of a \fmiGet is amortised among those child nodes. Hence, even if for some model the average time of a \fmiGet is high because the operation is inefficient, the term $\frac{1}{\avgBranch}\fmiGet$ of \cref{eq:speed-up-simple} becomes negligible. In \cref{sec:results:perf:preliminary} we show that our assumptions that motivate this remark are reasonable for a large set of benchmark models.

\begin{figure}
\centering
\hfill
\begin{subfigure}{\FigureTwoCols}
  \IncludeGraphics[width=\linewidth]{figures-limit-100.pdf}
  \caption{}
  \label{fig:limit-100}
\end{subfigure}
\hfill
\begin{subfigure}{\FigureTwoCols}
  \IncludeGraphics[width=\linewidth]{figures-limit.pdf}
  \caption{}
  \label{fig:limit-10-100}
\end{subfigure}
\hfill
\label{fig:limit}
\caption{Threshold $\speedupthreshold{\maxHeight}{\avgBranch}$ computed for $\maxHeight = 100$ (a) and for different values of $\maxHeight$ (b). In the right figure (b), our threshold is also normalised by $\maxHeight - 1$ for presentation purposes.}
\end{figure}

In \cref{fig:limit-100} we show that, starting from small values of \avgBranch, the threshold \speedupthreshold{\maxHeight}{\avgBranch} rapidly reaches values towards the limit $\maxHeight - 1$.
This is true also for different values of $\maxHeight$ as \cref{fig:limit-10-100} shows.

Hence, under our assumptions, given an \Ac{FMU} and a tree having a low branching factor, namely 4-5,
if the average execution time needed to perform a \fmiSet operation is lower than the time to perform a simulation of a scenario of length $\maxHeight-1$, then
% 
the speed-up of a \optimisedSearch \wrt a \traditionalSearch is greater than 1.

In \cref{sec:results:performance}, we present experimental results regarding the speed up computation on different \Acp{FMU} by taking into account trees of different depths and branching factors.




==> 20-methods-validation.tex <==
%!TEX  root=root.tex
%
\begin{figure}
  \Input{figures-simpath.tex}
  \caption{A glimpse of our strategy to evaluate correctness.}
  \label{fig:validation}
\end{figure}
%
To validate our methods to get and set complete \Ac{FMU} states, we have to check that a call to \fmiSet correctly replaces the current \Ac{FMU} state with an \Ac{FMU} state obtained by a previous call to \fmiGet.
To do so, we need to verify that further simulations are correctly computed accordingly to the actual \Ac{FMU} state.  



In particular, we define the following two ways of performing a simulation of an input \Ac{FMU}.


Given an \Ac{FMU}
and a value $\tau \in \RealsGEZ$,
let $s$ be the current state of the input \Ac{FMU},
we denote with $s' = \simulate{\tau}$ a function that simulates the input \Ac{FMU} advancing its current state $s$ for $\tau$ time units and reaching the state $s'$. 



Given an \Ac{FMU}
and values $\tau \in \RealsGEZ$, $\tau' \in \RealsGEZ$,
let $s$ be the current state of the input \Ac{FMU},
we denote with $s' = \simulatemod{\tau}{\tau'}$ a function that executes the following instructions:
\begin{enumerate}
    \item \fmiGetArgs{s};
    \item \simulate{\tau'};
    \item \fmiSetArgs{s};
    \item $s' \leftarrow \simulate{\tau}$.
\end{enumerate}
For the sake of readability and without loss of generality, we omit the call to \fmiFreeExtended in the above instructions as its correctness does not affect our validation process.

Intuitively, a call to \simulatemod{\tau}{\tau'}, for any $\tau' \in \RealsGEZ$, is semantically equivalent to a call to \simulate{\tau}, since they both advance the current \Ac{FMU} state for $\tau$ units of time.
This leads to the following remarks.

\begin{restatable}{remark}{remarksamestate}
Given an \Ac{FMU}
and a value $\tau \in \RealsGEZ$
let $s$ be the current state of the input \Ac{FMU}.
Then for all $\tau' \in \RealsGEZ$,
\simulate{\tau} and \simulatemod{\tau}{\tau'} reach exactly the same state, formally $\simulate{\tau} = \simulatemod{\tau}{\tau'}$
\end{restatable}

\begin{restatable}{remark}{remarksamesequence}
Given an \Ac{FMU}
and a value $\tau \in \RealsGEZ$,
let $s$ be the initial state of the input \Ac{FMU},
let \stateseqdef{\tau}%{\simHorizon}
and
\stateseqmoddef{\tau}%{\simHorizon}
be the sequences of \Ac{FMU} states reachable from $s$ by consecutive executions of \simulate{\tau} and \simulatemod{\tau}{\tau'}, respectively, for all $\tau' \in \RealsGEZ$.
If both \fmiGet and \fmiSet are implemented correctly then,
for all $i \in \{0, \ldots, n\}$, 
$s_i = s^*_i$.
\end{restatable}



To experimentally verify the above statement, we need to check that our implementation works for all values of $\tau'$. This is of course impossible. To overcome such an obstacle we employ a statistical approach based on hypothesis testing where $\tau'$ takes values in a bounded interval $\mathbb{B} \subset \RealsGEZ$ (see, \eg~\cite{grosu-etal:2005:tacas,mancini-etal:2018:smartgridcomm,mancini-etal:2015:iwbbio}).


Given a value for $\varepsilon \in (0,1)$, we define a \emph{null hypothesis} $H_0$ which states that
the probability of sampling $\tau' \in \mathbb{B}$ such that the state reached by executing $\simulate{\tau}$ is different from the state reached by executing $\simulatemod{\tau}{\tau'}$ is greater than $\varepsilon$.
Formally $H_0$ is defined as: $H_0 : \Pr\{\tau' \in \mathbb{B} \,.\, \simulate{\tau} \neq \simulatemod{\tau}{\tau'}\} \geq \varepsilon$.

Then we apply statistical hypothesis testing~\cite{mood:1974:statistics} and try to reject $H_0$ through a given number of trials $N$.

At each trial we randomly sample a value of
$\tau' \in \mathbb{B}$ according to a uniform distribution and we check whether the state reached by $\simulate{\tau}$ is different from the state reached by $\simulatemod{\tau}{\tau'}$ or not.

If within $N$ trials we find a value $\tau'$ such that $\simulate{\tau} \neq \simulatemod{\tau}{\tau'}$, then $\tau'$ is a counterexample showing that our implementation is not correct. Formally, we prove $H_0$ when it holds.

On the other hand, rejecting $H_0$ after $N$ trials, even if it holds, introduces a \emph{Type-I Error}.

In particular, given a value $\delta \in (0,1)$, the probability that we make an error by rejecting $H_0$ when it holds is bounded by $\delta$.

This is shortly stated by saying that $H_0$ is rejected with statistical confidence $1-\delta$.
Finally, we conclude that
the probability to sample $\tau'$ such that the state reached by executing $\simulate{\tau}$ is different from the state reached by executing $\simulatemod{\tau}{\tau'}$ is less than $\varepsilon$, formally $\Pr\{\tau' \in \mathbb{B} \,.\, \simulate{\tau} \neq \simulatemod{\tau}{\tau'}\} < \varepsilon$.

By exploiting results of~\cite{grosu-etal:2005:tacas}, given $\delta \in (0,1)$ and $\varepsilon \in (0,1)$, the number of trials is computed as $N = \lceil \log{(\delta)} / \log{(1 - \varepsilon)} \rceil$.

\Input{20-methods-algo-content.tex}

\Cref{algo:correctness} describes our \emph{Hypothesis Testing} approach and \Cref{fig:validation} sketches our correctness evaluation strategy.

Note that at Line \ref{algo:line:neq} of \cref{algo:correctness}, if, for a given $\tau'$, $\simulate{\tau} \neq \simulatemod{\tau}{\tau'}$ is true, we return such a $\tau'$ as a counterexample meaning that 
by simulating the input \Ac{FMU} $i$ times we reach a state proving that \fmiGet and \fmiSet are not working correctly.

The above considerations prove the following theorem. 
\begin{theorem}
\label{thm:algo}
Given an \Ac{FMU} having \fmiGet and \fmiSet implemented, values $\varepsilon, \delta \in (0,1)$, a bounded interval $\mathbb{B} \subset \RealsGEZ$ and a value for $\tau \in \RealsGEZ$,
\cref{algo:correctness} is such that:
\begin{enumerate}
    \item it terminates in $N$ steps, where $N = \left\lceil\frac{\log{(\delta)}}{\log{(1-\varepsilon)}}\right\rceil$;
    \item when it returns \texttt{True}, with confidence $1-\delta$: $\Pr\{\tau' \in \mathbb{B} \,.\, \simulate{\tau} \neq \simulatemod{\tau}{\tau'}\} < \varepsilon$;
    \item when it returns \texttt{False}, we have a counterexample, \ie a value for $\tau' \in \mathbb{B}$, proving that \fmiGet and \fmiSet are not correctly implemented.
\end{enumerate}
\end{theorem}

In \Cref{sec:results:validation} we apply \cref{algo:correctness} on different \Acp{FMU} in order to validate our implementation of \fmiGet and \fmiSet.


==> 30-results-case-studies.tex <==
%!TEX root = root.tex
%
In \cref{sec:results:performance} we see that, depending on the \Ac{FMU} at hand, different components of the \Ac{FMU} architecture are involved during saving and restoring an \Ac{FMU} state.

To assess correctness and to evaluate performance on all such components we evaluate our implementation by using
\Acp{FMU} generated from the following widely established model libraries.
\begin{description}
\item[\Ac{MSL}:]
the official Modelica library collecting models that are developed and reviewed by the Modelica Association (version 3.2.2, \url{https://modelica.org}).
It provides models and components from different engineering domains such as mechanical, electrical, magnetic, fluid, thermal and control systems.
The library contains both models defining standardised interfaces or building blocks and models that are directly usable.
For our purpose, we focus on the latter class of models, which comprises \DataGet{exps/msl/models} models having \DataGet{exps/msl/models/variables/avg} model variables on average.
% \end{Section}
%
% \begin{Section}{\Acl{STS}}
\item[\Ac{STS}:]
a Modelica library of benchmark models useful for assessing performance of large scale systems~(version 1.11.4, see~\cite{casella:2015:modelica}).
The library contains 16 models covering electrical, mechanical, power and thermal domains. Such models are scalable in terms of their size (\ie number of variables).
The \Ac{STS} provides also \DataGet{exps/sts/models} ready-to-run models validated by the authors and having an average of \DataGet{exps/sts/models/variables/avg} model variables.
% \end{Section}
%
\item[\Ac{BMD}:]
a well-known repository of mathematical models of biological systems taken from the scientific literature~\cite{lenovere-etal:2006:biomodels}.
A subset of these models, consisting of manually curated models, is widely-used as a benchmark for \Ac{SBML} simulators.
From such a subset, we used models already translated from \Ac{SBML} to Modelica and validated in~\cite{maggioli-etal:2019:bioinf}. In total we consider \DataGet{exps/bmd/models} models having \DataGet{exps/bmd/models/variables/avg} model variables on average.
\end{description}

\begin{figure}
\centering
\hfill
\begin{subfigure}{\FigureThreeCols}
  \IncludeGraphics[width=\linewidth]{figures-msl-distribution.pdf}
  \caption{}
  \label{fig:models:msl}
\end{subfigure}
\hfill
\begin{subfigure}{\FigureThreeCols}
  \IncludeGraphics[width=\linewidth]{figures-sts-distribution.pdf}
  \caption{}
  \label{fig:models:sts}
\end{subfigure}
\hfill
\begin{subfigure}{\FigureThreeCols}
  \IncludeGraphics[width=\linewidth]{figures-bmd-distribution.pdf}
  \caption{}
  \label{fig:models:bmd}
\end{subfigure}
\hfill
\caption{Distribution of sizes of models within \Ac{MSL} (a), \Ac{STS} (b) and \Ac{BMD} (c).}
\label{fig:models}
\end{figure}


\cref{fig:models} shows the distribution of model sizes in terms of the number of model variables.


==> 30-results-content.tex <==
%!TEX root = ../root.tex
In this section, we present experimental results to evaluate
the correctness and the effectiveness of our implementation against state-of-the-art case studies.
After briefly describing such case studies, we evaluate correctness 
and we finally show how our implementation enhances performance of simulation-based \Ac{VV} approaches.

\subsection{Case studies}
\label{sec:casestudies}
\Input{30-results-case-studies.tex}
%
\subsection{Experimental setting}
\label{sec:results:setting}
\Input{30-results-settings.tex}
%
\subsection{Correctness evaluation results}
\label{sec:results:validation}
\Input{30-results-validation.tex}
%
\subsection{Performance evaluation results}
\label{sec:results:performance}
\Input{30-results-evaluation.tex}


==> 30-results-evaluation.tex <==
%!TEX root=./root.tex
%
In this section, we describe experimental results of our performance evaluation according to our strategy described in \cref{sec:performance}.
In particular, in \cref{sec:results:perf:preliminary} we evaluate performance of our implementation by a preliminary analysis using results of \cref{remark:limit}. Then, in \cref{sec:results:perf:speed-up} we compute the speed-up of a \optimisedSearch \wrt a \traditionalSearch on trees with different values of depth and branching factor. 

\subsubsection{Preliminary analysis}%
\label{sec:results:perf:preliminary}%
As a preliminary analysis, for each \Ac{FMU}, we computed the ratio \setsimratio (see \cref{remark:limit}) to compare
the execution time of a \fmiSet with the execution time needed for simulating the given \Ac{FMU}.


Such an analysis has been conducted by 
taking into account different values for the depth of the tree, \ie $\maxHeight \in
\left[\DataGet{exps/fmu/h/min}, \DataGet{exps/fmu/h/max}\right]$.

\begin{figure}[!htp]
\centering
\hfill
\begin{subfigure}{\FigureOneCol}
  \IncludeGraphics[width=0.55\linewidth]{figures-msl-scatter.pdf}
  \caption{}
  \label{fig:simtime:average:msl}
\end{subfigure}
\hfill
\begin{subfigure}{\FigureOneCol}
  \IncludeGraphics[width=0.55\linewidth]{figures-sts-scatter.pdf}
  \caption{}
  \label{fig:simtime:average:sts}
\end{subfigure}
\hfill
\begin{subfigure}{\FigureOneCol}
  \IncludeGraphics[width=0.55\linewidth]{figures-bmd-scatter.pdf}
  \caption{}
  \label{fig:simtime:average:bmd}
\end{subfigure}
\hfill
\caption{Correlation among the execution times (in seconds) of a simulation of duration $\maxHeight \times \tau$ (on x axis) and $\maxHeight$ simulations of duration $\tau$ (on y axis), where $h = \DataGet{exps/fmu/h/max}$. Each marker represents an \Ac{FMU} within \Ac{MSL} (a), \Ac{STS} (b) and \Ac{BMD} (c).} 
\label{fig:simtime:average}
\end{figure}
%
\begin{figure}[!htp]
\centering
\hfill
\begin{subfigure}{\FigureOneCol}
  \IncludeGraphics[width=0.6\linewidth]{figures-msl-time-set.pdf}
  \caption{}
  \label{fig:time-set:msl}
\end{subfigure}
\hfill
\begin{subfigure}{\FigureOneCol}
  \IncludeGraphics[width=0.6\linewidth]{figures-sts-time-set.pdf}
  \caption{}
  \label{fig:time-set:sts}
\end{subfigure}
\hfill
\begin{subfigure}{\FigureOneCol}
  \IncludeGraphics[width=0.6\linewidth]{figures-bmd-time-set.pdf}
  \caption{}
  \label{fig:time-set:bmd}
\end{subfigure}
\hfill
\caption{Execution times (in seconds) spent for performing \fmiSet during \Ac{FMU} simulations. Each line represents an \Ac{FMU} within \Ac{MSL} (a), \Ac{STS} (b) and \Ac{BMD} (c).} 
\label{fig:time-set}
\end{figure}
%
To perform such an analysis we show that our assumptions (\ie those described in \cref{sec:opt-search}) are reasonable for our case-study \Acp{FMU}.
To do so, in \cref{fig:simtime:average}, we compared the execution time of a simulation of length
$i\times\tau$ with the execution time of $i$ simulations of length $\tau$.
As we see, these two quantities are highly correlated.
Indeed, the Pearson correlation coefficient, $\rho$, for \Ac{MSL}, \Ac{STS} and \Ac{BMD} is \DataGet{exps/simtime/msl/rho}, \DataGet{exps/simtime/sts/rho} and \DataGet{exps/simtime/bmd/rho}, respectively.

Moreover, in \cref{fig:time-set}, for each \Ac{FMU}, we show that the execution time (in seconds) spent to perform a \fmiSet operation is almost constant during the \Ac{FMU} simulation (from its start time to its simulation horizon).

There is also an atypical behaviour for two \Acp{FMU} within \Ac{BMD}. In such models, the
\texttt{delay} operator is used and  
parameter \texttt{tmax} is always set to be as large as possible (much larger than the given \Ac{FMU} simulation horizon).
This causes the size of the associated delay buffers to increase after each simulation in order to store all needed delay variable values.
For this reason, the size of the internal \Ac{FMU} state also increases together with the execution time needed to perform \fmiSet (and also \fmiGet as well).

\begin{figure}[!htp]
\centering
\hfill
\begin{subfigure}{\FigureOneCol}
  \IncludeGraphics[width=0.6\linewidth]{figures-msl-setsim.pdf}
  \caption{}
  \label{fig:setsim:msl}
\end{subfigure}
\hfill
\begin{subfigure}{\FigureOneCol}
  \IncludeGraphics[width=0.6\linewidth]{figures-sts-setsim.pdf}
  \caption{}
  \label{fig:setsim:sts}
\end{subfigure}
\hfill
\begin{subfigure}{\FigureOneCol}
  \IncludeGraphics[width=0.6\linewidth]{figures-bmd-setsim.pdf}
  \caption{}
  \label{fig:setsim:bmd}
\end{subfigure}
\hfill
\caption{Computation of \setsimratio, where $\maxHeight \in \left[\DataGet{exps/fmu/h/min}, \DataGet{exps/fmu/h/max}\right]$. Dashed lines represent thresholds of \setsimratio. Each curve represents an \Ac{FMU} within \Ac{MSL} (a), \Ac{STS} (b) and \Ac{BMD} (c).}
\label{fig:setsim}
\end{figure}

Having clarified that our assumptions are reasonable, in \cref{fig:setsim}
we show how \setsimratio changes by varying the depth of the tree, for each \Ac{FMU} in our datasets.

As we expected, for the majority of the analysed \Acp{FMU}, the values of \setsimratio are either below 1 or they go below 1 for very small values of depth (namely, $<20$).
This means that the cost of \fmiSet is very low \wrt simulations in terms of computation time.

Also, there is one single \Ac{FMU} having \setsimratio greater than 1 for all values of depth.
Such behaviour is explained by the fact that the larger the state of a given \Ac{FMU} the slower the execution of \fmiSet in terms of computation time.
Hence, a \traditionalSearch performs better for those \Acp{FMU} having a very large state (thousands of variables, as for \Acp{FMU} within \Ac{STS}) but very fast in simulating.
Of course, as we described in \cref{sec:opt-search}, this is strictly linked also to the depth of the given tree which affects the length of simulations to be performed in a \traditionalSearch.

Note that, \setsimratio is less than 1 also for those two \Acp{FMU} having a non-constant execution time for \fmiSet (see \cref{fig:time-set:bmd}).

\subsubsection{Speed-up analysis}
\label{sec:results:perf:speed-up}
%
In order to perform a more in-depth analysis, we also computed our cost functions for the \traditionalSearch, \ie \cref{eq:cost-trad}, and the \optimisedSearch, \ie \cref{eq:cost-opt}, and finally our speed-up formula, \ie \speedup{\maxHeight}{\avgBranch} (see \cref{eq:speed-up}).

To do so, different values for the branching factor,
\ie $\avgBranch \in
\left[\DataGet{exps/fmu/b/min}, \DataGet{exps/fmu/b/max}\right]$,
and for the depth of the tree,
\ie $\maxHeight \in
\left[\DataGet{exps/fmu/h/min}, \DataGet{exps/fmu/h/max}\right]$, have been taken into account.
Note that, such chosen values are perfectly reasonable for real case studies.
For example, in~\cite{mancini-etal:2018:rcra-treatment,sinisi-etal:2020:fundamenta}
a simulation-based approach consisting in a backtracking-based search has been employed in a search space defined as a tree of depth equal to $55$ and constant branching factor equal to $3$.

\begin{figure}[!htp]
\centering
\hfill
\begin{subfigure}{\FigureOneCol}
  \IncludeGraphics[width=0.6\linewidth]{figures-msl-performance-3d.pdf}
  \caption{}
  \label{fig:speedup:msl}
\end{subfigure}
\hfill
\begin{subfigure}{\FigureOneCol}
  \IncludeGraphics[width=0.6\linewidth]{figures-sts-performance-3d.pdf}
  \caption{}
  \label{fig:speedup:sts}
\end{subfigure}
\hfill
\begin{subfigure}{\FigureOneCol}
  \IncludeGraphics[width=0.6\linewidth]{figures-bmd-performance-3d.pdf}
  \caption{}
  \label{fig:speedup:bmd}
\end{subfigure}
\hfill
\caption{Average speed-up (heat map) computed among \Acp{FMU} within \Ac{MSL} (a), \Ac{STS} (b) and \Ac{BMD} (c) by varying the branching factor and the depth of the tree.}
\label{fig:speedup}
\end{figure}


\Cref{fig:speedup} shows
the average speed-up computed among \Acp{FMU} within
\Ac{MSL}, \Ac{STS} and \Ac{BMD}
when varying both the branching factor and the depth of the tree.

As we expected from our preliminary analysis (\cref{sec:results:perf:preliminary}),
even with a low value for the branching factor, \ie 5, and a low depth, \ie 50, a \optimisedSearch is, on average,
$\TotalAvgSpeedup$ times faster than a \traditionalSearch, among all our case studies.
In particular, for \Acp{FMU} within \Ac{MSL}, \Ac{STS} and \Ac{BMD}, we have on average a speed-up of
$\TotalAvgSpeedupMSL$, $\TotalAvgSpeedupSTS$ and $\TotalAvgSpeedupBMD$, respectively.

Furthermore, by keeping constant the given tree depth and branching factor, $\maxHeight = \DataGet{exps/fmu/h/max}$ and $\avgBranch = \DataGet{exps/fmu/b/max}$, we reach, on average, a speed-up value of $\TotalMaxSpeedupMSL$, $\TotalMaxSpeedupSTS$ and $\TotalMaxSpeedupBMD$, among all \Acp{FMU} within \Ac{MSL}, \Ac{STS} and \Ac{BMD}, respectively.

As we can note, \Acp{FMU} within \Ac{BMD} (\cref{fig:speedup:bmd}) achieve higher values of speed-up than \Acp{FMU} within the other datasets.
It is clear (starting from depth equal to 2) that the execution time of \fmiSet is very low \wrt simulation execution time. Hence, the deeper the tree (\ie the number of simulations) higher the speed-up achieved.

Surprisingly, as \cref{fig:speedup:msl} shows, for some values of \maxHeight the computed speed-up is around $70$.
This behaviour is due to the fact that, for some \Acp{FMU} within \Ac{MSL} the numerical integrator reaches a computationally expensive integration step which requires more time to be solved, \eg a chattering effect.

Hence, having the \Ac{FMU} at hand equipped with \fmiGet and \fmiSet functionalities brings a huge benefit.
Indeed, once this complex integration step is solved, the reached \Ac{FMU} state can be saved and restored for further simulations.

\begin{figure}[!htp]
\centering
\hfill
\begin{subfigure}{\FigureOneCol}
  \IncludeGraphics[width=0.6\linewidth]{figures-msl-performance-b-10.pdf}
  \caption{}
  \label{fig:speedup-10:msl}
\end{subfigure}
\hfill
\begin{subfigure}{\FigureOneCol}
  \IncludeGraphics[width=0.6\linewidth]{figures-sts-performance-b-10.pdf}
  \caption{}
  \label{fig:speedup-10:sts}
\end{subfigure}
\hfill
\begin{subfigure}{\FigureOneCol}
  \IncludeGraphics[width=0.6\linewidth]{figures-bmd-performance-b-10.pdf}
  \caption{}
  \label{fig:speedup-10:bmd}
\end{subfigure}
\hfill
\caption{Speed-up achieved for each \Ac{FMU} within \Ac{MSL} (a), \Ac{STS} (b) and \Ac{BMD} (c) when the branching factor is equal to $\DataGet{exps/fmu/b/max}$ and the depth takes values within $\left[\DataGet{exps/fmu/h/min}, \DataGet{exps/fmu/h/max}\right]$.}
\label{fig:speedup-10}
\end{figure}

\Cref{fig:speedup-10} clearly shows this by presenting, for each evaluated \Ac{FMU}, the speed-up achieved when varying the depth of the tree, while keeping constant the value of the branching factor ($\avgBranch = \DataGet{exps/fmu/b/max}$).
In particular, in \cref{fig:speedup-10:msl} we see that few \Acp{FMU} reach peaks of speed-up above $10\,000$.

Furthermore, in both \cref{fig:speedup,fig:speedup-10}, we note that the speed-up increases almost linearly \wrt values of the depth of the tree.



==> 30-results-settings.tex <==
%!TEX root=./root.tex
%
All our experiments have been carried out on a \Ac{HPC} infrastructure (\ie Marconi cluster at CINECA, Italy).

For each Modelica model within our datasets, \ie \Ac{MSL}, \Ac{STS} and \Ac{BMD}, we generated its \Ac{FMU} using our extended \JModelica.

We manually excluded from our datasets those \Acp{FMU} that are not compatible with get/set state functionality. These are \Acp{FMU} that use external objects (as described in \cref{sec:state-architecture}).
This led us to exclude
\Pretty{\mslFMUnotpass} (\ie \Pretty{\MSLnotpassPerc}\%) models from \Ac{MSL} and \Pretty{\stsFMUnotpass} (\ie \Pretty{\STSnotpassPerc}\%) models from \Ac{STS}.
All models within \Ac{BMD} have been included. 
Hence, in total, we excluded the \Pretty{\totalFMUnotpassPerc}\% of all \Acp{FMU} within our datasets.


In order to assess correctness and evaluate performance of our implementation of get/set functionality, \Acp{FMU} have been simulated using \texttt{SUNDIALS} \texttt{CVODE}~\cite{hindmarsh2005sundials} solver by means of the \texttt{PyFMI} library~\cite{andersson2016pyfmi}.
For each \Ac{FMU}, we set the value of $\tau$ to \valueTau\% of the \Ac{FMU} default simulation horizon, \ie the value of \Ac{FMU} \texttt{default experiment stop time}.


==> 30-results-validation.tex <==
%!TEX  root=root.tex
%
%
%
%
%
Correctness has been evaluated by means of the approach presented in \cref{sec:validation}.
In particular, for each of the \Pretty{\totalFMUpass} \Acp{FMU}, we ran our \cref{algo:correctness} to assess that our implementation correctly restores a previously-saved \Ac{FMU} state.

To do so, we consider as $\mathbb{B}$ values from 0 to the default simulation horizon of the given \Ac{FMU} and we set $\delta = 8\%$ and $\varepsilon = 2.5\%$.
Thus the number of trials has been set to $N = 100$.

During the sampling process,
the inequality of \Ac{FMU} states (Line \ref{algo:line:neq} of \cref{algo:correctness}) has been checked through a bit-wise comparison.
For all our \Pretty{\totalFMUpass} \Acp{FMU} our \cref{algo:correctness} returned true, proving that our implementation is correct with a degree of statistical confidence of $92\%$.


==> 40-conclusions-content.tex <==
%!TEX  root=root.tex
%
We have presented an extended version of \JModelica that implements \Ac{FMI} 2.0 methods to save and restore complete states of \Acp{FMU} for \Ac{ME}.
We have conducted an in-depth evaluation of our implementation on \Acp{FMU} generated from widely established model libraries, namely \Ac{MSL}, \Ac{STS} and \Ac{BMD}.
We have shown the correctness of our proposed implementation and assessed its performance on a demanding application such as simulation-based \Ac{VV} approaches that drive the input \Ac{FMU} in the space of all simulation scenarios.
In doing so, we computed the speed-up of a visit which
drives \Acp{FMU} generated by our extended \JModelica implementation \wrt a visit which drives \Acp{FMU} generated by stand-alone \JModelica.
We have shown even for a tree with a low branching factor, namely $5$, and a low depth, namely $50$, the speed-up achieved is, on average, $\TotalAvgSpeedupMSL$, $\TotalAvgSpeedupSTS$ and $\TotalAvgSpeedupBMD$, among all \Acp{FMU} within \Ac{MSL}, \Ac{STS} and \Ac{BMD}, respectively. Also, the achieved speed-up increases much more for deeper trees.
Future directions can be to apply our save-and-restore implementation to \Acp{FMU} for \Ac{CS} as well as to port our implementation to the OpenModelica simulation environment. Moreover, as the 3.0 version of \Ac{FMI} standard is planned to be released, it could be worth investigating how to adapt and extend our implementation to the new set of envisioned features (\eg clocks and hybrid co-simulation to handle event-driven dynamics and a new type of model exchange format, \ie Scheduled Execution, SE). 



==> abstract.tex <==
%!TEX  root=root.tex
%
A \Ac{CPS} comprises physical as well as software subsystems.
Simulation-based approaches are typically used to support design and \Ac{VV} of \Acp{CPS} in several domains such as: aerospace, defence, automotive,
smart grid and healthcare.

Accordingly, many simulation-based tools are available to support \Ac{CPS} design.
This, on one side, enables designers to choose the toolchain that best suits their needs, on the other side poses huge interoperability challenges when one needs to simulate \Acp{CPS} whose subsystems have been designed and modelled using different toolchains.
To overcome such an interoperability problem, in 2010 the \Ac{FMI} has been proposed as an open standard to support both \Ac{ME} and \Ac{CS} of simulation models created with different toolchains.
\Ac{FMI} has been adopted by several modelling and
simulation environments.
Models adhering to such a standard are called \Acp{FMU}. Indeed \Acp{FMU} play an essential role in defining complex
\Acp{CPS} through, \eg the \Ac{SSP} standard.

Simulation-based \Ac{VV} of \Acp{CPS} typically requires exploring different simulation scenarios (\ie exogenous input sequences to the \Ac{CPS} under design).
Many such scenarios have a shared prefix.
Accordingly, to avoid simulating many times such shared prefixes, the simulator state at the end of a shared prefix is saved and then restored and used as a start state for the simulation of the next scenario.
In this context, an important \Ac{FMI} feature is the capability to save and restore the internal \Ac{FMU} state on demand. This is crucial to increase efficiency of simulation-based \Ac{VV}.
Unfortunately, the implementation of this feature is not mandatory
and it is available only within some commercial software.
As a result, the interoperability enabled by the \Ac{FMI} standard cannot be fully exploited for \Ac{VV} when using open-source simulation environments.
This motivates developing such a feature for open-source \Ac{CPS} simulation environments.

Accordingly, in this paper, we focus on \JModelica, an open-source modelling and simulation environment for \Acp{CPS} based on an open standard modelling language, namely Modelica.
We describe how we have endowed \JModelica
with
our open-source
implementation of the \Ac{FMI} 2.0 functions needed
to save and restore internal states of \Acp{FMU} for \Ac{ME}.
Furthermore, we present experimental results evaluating, through $\totalFMUpass$ benchmark models, correctness and efficiency of our extended \JModelica.
Our experimental results show that simulation-based \Ac{VV} is, on average, $\TotalAvgSpeedup$ times faster with our get/set functionality than without it.



==> content.tex <==
%!TEX root = ./root.tex
% 
% 
\AcronymResetAll
%
\section{Introduction}%
\AcronymResetAll%
\label{sec:intro}%
\Input{10-introduction-content.tex}%
% 
\section{Related Work}%
\AcronymResetAll%
\label{sec:related-work}%
\Input{15-related-work-content.tex}%
%
\section{Methods}%
\AcronymResetAll%
\label{sec:methods}%
\Input{20-methods-content.tex}
% 
\section{Experimental Results}%
\AcronymResetAll%
\label{sec:results}%
\Input{30-results-content.tex}%
%
\section{Conclusions}%
\AcronymResetAll%
\label{sec:conclusions}%
\Input{40-conclusions-content.tex}%
% 
\section*{Acknowledgements}%
%
The authors are grateful to their alumni, Agostina Calabrese, Michele Laurenti, and Alessandro Steri, for their contribution to develop a first prototype during their bachelor thesis work.


This work was partially supported by the following research projects and grants: 
%
Italian Ministry of University \& Research (MIUR) grant ``Dipartimenti di Eccellenza 2018--2022'' (Dept.\ Computer Science, Sapienza Univ.\ of Rome); 
EC FP7 project PAEON (Model Driven Computation of Treatments for Infertility Related Endocrinological Diseases, 600773);
EC FP7 project SmartHG (Energy Demand Aware Open Services for Smart Grid Intelligent Automation, 317761);
Sapienza University 2018 project RG11816436BD4F21 ``Computing Complete Cohorts of Virtual Phenotypes for In Silico CLinical Trials and Model-Based Precision Medicine'';
A system for UAV detection (Aerospace and security,POR FESR 2014-2020);
INdAM ``GNCS Project 2020'';
CINECA Class C ISCRA Project (HP10CPJ9LW).


\bibliographystyle{elsarticle-num}
\bibliography{biblio}

\clearpage

\appendix
\section{Proof of Results}
\label{appendix}
\Input{90-appendix-content.tex}
\section{Software}
\label{appendix-software}
Our extended \JModelica \JModelicaVersion is publicly available at \RepoUrl\\

Software tools used for evaluating correctness and performance of our implementation are available at \url{https://bitbucket.org/mclab/getsetfmustateeval}


==> figures-cost.tex <==
%!TEX root = root.tex

\begin{tikzpicture}[>=latex]
  \node[draw,shape=circle] (s) {$s_{i-1}$};
  \node[] (prefix) [above=of s] {};
  \draw[->,decorate,decoration=snake] (prefix) -- (s);
  \node[node distance=0.2cm] (get) [left=of s] {\fmiGetArgs{s_{i-1}}};
  \node[] (dots) [below=of s] {\ldots};
  \draw[->] (s) to node [auto] {$\Vector{u}_k$} (dots);
  \node[draw,shape=circle] (left) [left=of dots] {};
  \node[align=left,node distance=0.2cm] [left=of left] {\fmiSetArgs{s_{i-1}}\\\simulate{\tau}};
  \draw[->] (s) to node [auto,swap] {$\Vector{u}_1$} (left);
  \node[draw,shape=circle] (right) [right=of dots] {};
  \node[align=left,node distance=0.2cm] [right=of right] {\fmiSetArgs{s_{i-1}}\\\simulate{\tau}};
  \draw[->] (s) to node [auto] {$\Vector{u}_{\avgBranch}$} (right);
  \draw[decorate,decoration={brace,mirror,amplitude=10pt,raise=5pt}] (left) -- (right);
  \node[node distance=0.4cm] (branching) [below=of dots] {\avgBranch};
\end{tikzpicture}


==> figures-fmu.tex <==
%!TEX root=./root.tex
\begin{tikzpicture}[thick,scale=0.7, every node/.style={scale=.6},>=latex]
  \node[draw,shape=circle] (s0) {$x(0)=1.0$};
  % \node[] (prefix) [above=of s] {};
  % \draw[->,decorate,decoration=snake] (prefix) -- (s);
  % \node[node distance=0.2cm] (s0_d) [left=of s0] {};
  \node[] (a) [below=of s0] {};
  % \draw[->] (s) to node [auto] {$\Vector{u}_k$} (dots);
  \node[draw,shape=circle] (s1) [left=of a] {$x(T)=0.3$};
  % \node[align=left,node distance=0.2cm] [left=of left] {\fmiSetArgs{s_{i-1}}\\\simulate{\tau}};
  \draw[->] (s0) to node [auto,swap] {$-1$} (s1);
  \node[draw,shape=circle] (s2) [right=of a] {$x(T)=2.7$};
  % \node[align=left,node distance=0.2cm] [right=of right] {\fmiSetArgs{s_{i-1}}\\\simulate{\tau}};
  \draw[->] (s0) to node [auto] {$1$} (s2);
  % \draw[decorate,decoration={brace,mirror,amplitude=10pt,raise=5pt}] (left) -- (right);
  % \node[node distance=0.4cm] (branching) [below=of dots] {\avgBranch};
  \node[] (aa) [below=of s1] {};
  \node[] (aaa) [below=of s2] {};
  \node[draw,shape=circle,node distance=0.3] (s3) [left=of aa] {$x(2T)=0.1$};
  \draw[->] (s1) to node [auto,swap] {$-1$} (s3);
  \node[draw,shape=circle,node distance=0.2] (s4) [right=of aa] {$x(2T)=1.0$};
  \draw[->] (s1) to node [auto] {$1$} (s4);
  \node[draw,shape=circle,node distance=0.2] (s5) [left=of aaa] {$x(2T)=1.0$};
  \draw[->] (s2) to node [auto,swap] {$-1$} (s5);
  \node[draw,shape=circle,node distance=0.3] (s6) [right=of aaa] {$x(2T)=7.3$};
  \draw[->] (s2) to node [auto] {$1$} (s6);

\end{tikzpicture}


==> figures-simpath.tex <==
%!TEX root = ../../root.tex

\begin{tikzpicture}[>=latex,state/.style={circle,draw,minimum size=10mm}]
  \node[] (prefix) {};
  \node[state] (spre) [right=of prefix] {$s_{i-1}$};
  \node[state,node distance=3cm] (s) [right=of spre] {$s_i$};
  \node[state,node distance=3cm] (snext) [right=of s]  {$s_{i+1}$};
  \node[state] (srandom) [below=of s]  {$s$};
  \node[] (end) [right=of snext] {};
  \draw[->,decorate,decoration=snake] (prefix) -- (spre);
  \draw[->,decorate,decoration=snake] (snext) -- (end);
  \draw[->] (spre) to node [auto] {\simulate{\tau}} (s);
  \draw[->] (s) to node [auto] {\simulate{\tau}} (snext);
  \draw[->] (s) [bend right=45] to node [auto,swap,align=right] {\fmiGetArgs{s_i}\\\simulate{\texttt{$\tau' \leftarrow$ rand()}}} (srandom);
  \draw[->] (srandom) [bend right=45] to node [auto,swap,align=left] {\fmiSetArgs{s_i}} (s);
\end{tikzpicture}


==> keywords.tex <==
Simulation\sep Verification and Validation\sep Interoperability\sep FMI/FMU\sep Model Exchange\sep Cyber-Physical Systems


==> title.tex <==
%!TEX root=./root.tex
%
% \title{FMI 2.0 full state \texttt{get} and \texttt{set} for JModelica FMUs}
\title{Reconciling interoperability with efficient Verification and Validation within open source simulation environments\tnoteref{t1}}
%
\author%[mainaddress]
{Stefano Sinisi\corref{correspondingauthor}}
\cortext[correspondingauthor]{Corresponding author}
\ead{sinisi@di.uniroma1.it}
%
\author%[mainaddress]
{Vadim Alimguzhin}
\author%[mainaddress]
{Toni Mancini}
\author%[mainaddress]
{Enrico Tronci}
%
\address%[mainaddress]
{Computer Science Department, Sapienza University of Rome, Italy}
%

\tnotetext[t1]{This article appears in Simulation Modelling Practice and Theory, 
Volume 109, May 2021, 102277. Elsevier. \url{https://doi.org/10.1016/j.simpat.2021.102277}}
